NFGen: Automatic Non-linear Function Evaluation Code Generator for General-purpose MPC Platforms

Due to the absence of a library for non-linear function evaluation, so-called general-purpose secure multi-party computation (MPC) are not as ''general'' as MPC programmers expect. Prior arts either naively reuse plaintext methods, resulting in suboptimal performance and even incorrect results, or handcraft ad hoc approximations for specific functions or platforms. We propose a general technique, NFGen, that utilizes pre-computed discrete piecewise polynomials to accurately approximate generic functions using fixed-point numbers. We implement it using a performance-prediction-based code generator to support different platforms. Conducting extensive evaluations of 23 non-linear functions against six MPC protocols on two platforms, we demonstrate significant performance, accuracy, and generality improvements over existing methods.

==> Makefile <==
PACKAGE=acmart

SAMPLES = \
	main.tex 

PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx
	pdflatex -synctex=1 -interaction=nonstopmode $<
	- bibtex $*
	pdflatex -synctex=1 -interaction=nonstopmode $<
	pdflatex -synctex=1 -interaction=nonstopmode $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -synctex=1 -interaction=nonstopmode $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex  ACM-Reference-Format.bst $(PACKAGE).cls
	pdflatex -synctex=1 -interaction=nonstopmode $<
	- bibtex $*
	pdflatex -synctex=1 -interaction=nonstopmode $<
	pdflatex -synctex=1 -interaction=nonstopmode $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -synctex=1 -interaction=nonstopmode $<; done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.pdf *.gz *.upa *.upb

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'



# Makefile for acmart package

# This file is in public domain

# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $


==> key.tex <==

\section{Challenges for Fixed-point Computation}
    In the field of numerical computation, real numbers are normally represented in the \textbf{Floating-point (FLP)} form. While for most MPC systems, the main number format representing real numbers are \textbf{Fixed-point (FXP)}. As the computation domain in MPC systems is normally discrete (\ie{ring or finite field}), they tend to embed each real number as an integer with a fixed resolution. For the non-linear function approximation task, the precision requirement about the numbers is very strict. Actually, most scientific computation libraries and applications like~\cite{virtanen2020scipy, harris2020array} are based on double-precision FLP. 
    
    The format and number representation logic are fundamentally different between FLP and FXP. How to  efficiently find an approximation in the FLP environment (\ie{traditional computation systems}) and at the same time maintaining its precision in the FXP environment (\ie{MPC systems}) evaluation is a difficult problem. This paper fills the gap between FLP and FXP environments by three techniques:
    1) \textit{data representation constraints} are forced during FLP computation, making sure the constructed value are within the range of FXP; 
    2) \textit{representaion magnification factor} is introduced to enlarge the representation range of FXP; 
    3) \textit{residual boosting}. The approximation procedure for each polynomial $p \in \mathcal{P}_{(k, m)}$ is multi-steps, with the objective changing from the original function $F$ to each residual error. Actually, each $p \in \mathcal{P}_{(k, m)}$ is the boosting result of less than $k-1$ polynomials, maximizing the approximation accuracy.
    
    
    In this section, we will first introduce the difference between FLP and FXP then illustrate the three techniques that play important roles in the precomputation phase.


    \para{Difference between FLP and FXP formats.  } FLP represent real numbers in three parts, 1) sign bit ($s = 1\, \text{or}\, 0$) 2) $e$-bit exponent and 3) $m$-bit mantissa (\textit{a.k.a, significand}), shown in Figure~\ref{Floating-point Format}. In IEEE 754 format, each real value $x \in \mathbb{R}$ are encoded as 
    \begin{equation}
        \text{FLP}(x) = (-1)^{s} \times (1.m_1m_2...m_{m})_2 \times 2^{E}
    \end{equation}
    where $s, m_1, m_2, ..., m_m$ are either 1 or 0, the exponent $E = (e_1e_2...e_e)_2 - (2^{e-1}-1)$, $(d_1d_2...d_n)_2$ means $n$-digit number in base 2. The range of exponent are $- 2^{e-1}-1 \leq E \leq 2^{e-1}$, lefting the all $1$ case for $\infty$ or \code{NaN}. In IEEE double precision floating-point formant, $e = 11$ and $m = 52$. For converience, all the $x \in \mathbb{R}$ in this paper means FLP($x$).

    FXP represent each real number in an $n$-bit integer with a fixed resolution $2^{-f}$, shown in Figure~\ref{Fixed-point Format}. The first bit is used for sign and others represent the value of the integer. In a $\langle n,f \rangle$ FXP representation systems, each real value $x \in \mathbb{R}$ are encoded as
    \begin{equation}
        \text{FXP}(x) = (-1)^{s} \times (d_2d_3...d_n)_2 \times 2^{-f}
    \end{equation}
    where $s, d_2 d_3, ... d_n$ are eigher 1 or 0. The role for resolution $2^{-f}$ played in FXP is like a fixed decimal point, spliting the $n-1$ value representaion bits into integer part (first $n-f-1$ bits) and fraction part (last $f$ bits).

    Both FLP or FXP formats are methods approximating real number $x \in \mathbb{R}$ in computers. The representation error inherently exists in both formats while there are enormous differences.
    1) From the precision perspective: FLP offers a definite $m$ significant bits corresponding to the number's exponent, while FXP is precious for fixed $f$ bits after the decimal point. Specifically, no matter how large or small the value $x$ is, FXP aims to offer a precious representation till $\log_{10}(2^{f})$ points after the decimal point, while the representable fractional points are changed in FLP format.
    2) From the range perspective: FLP offers a more broad range comparing with FXP even with less bits. For $64$-bit double precision FLP, the representable range are from $2^{-1023}$ to $2^{+1024}$; While for $128$-bit FXP, the range are only $2^{-(128-f-1)}$ to $2^{+(128-f-1)}$ ($f < 128$). 

    \begin{figure}[htb]
        \centering
        \subfigure[FLP Format]{
            \label{Floating-point Format}
            \includegraphics[width=0.45\textwidth]{./graph/FLP-format.pdf}
        }
        \subfigure[FXP Format]{
            \label{Fixed-point Format}
            \includegraphics[width=0.45\textwidth]{./graph/FXP-format.pdf}
        }
        \caption{Data Representation Formats}
    \end{figure}

    \para{1) \textit{Data Representation Constraints}.  } The task for constructing a polynomial approximation to a specific non-linear function $F$ is well-known computationally intensive. From both efficiency and accuracy perspectives, the approximation construction stage should be loaded on the long-developed scientific computation environments, which are mainly based on FLP. Aiming to maintain the precision of approximation in the online phase of FXP environments, we have to set a series of constraints to limit the power of FLP numbers. The constraints are adapted to the underlying $\langle n,f \rangle$ FXP systems as the precision and range vary. For any FLP encoded number $x$, we have the following rules to create a simulation of FXP in the FLP environment.

    \begin{itemize}
        \item $\mathsf{OverflowR}(x, n, f): $ Owing to avoid the overflow in FXP systems, $\mathsf{OverflowR}$ checks the absolute value $|x|$ with the maximum representable number $2^{n-f-1}$ in $\langle n,f \rangle$ FXP system, round the overflow part if it exceeds the representation range. 
            \begin{equation}
                \mathsf{OverflowR}(x, n, f) = \mathsf{sign}(x) \times \min{(|x|, 2^{n-f-1})}
            \end{equation} 
        \item $\mathsf{UnderflowR}(x, f): $ Owing to avoid the underflow in FXP systems, $\mathsf{UnderflowR}$ checks the absolute value $|x|$ with the minimum representable number $2^{-f}$ in $\langle n,f \rangle$ FXP system, round the underflow part off to zero.
            \begin{equation}
                \mathsf{UnderflowR}(x, f) = \mathsf{sign}(x) \times \max{(|x|, 2^{-f})}
            \end{equation}
        \item $\mathsf{FLPsimFXP}(x, f, n): $ For any real value $x \in \mathbb{R}$, even it is in the intersection of representation range of FLP and FXP, the real value changes significantly when we load $x$ from FLP to FXP environments. This is the problem that the precision varies between two environments. Not all the significand in FLP can be loaded into FXP systems. $\mathsf{FLPsimFXP}$ is used to round off the unrepresentable bits in specific FXP systems. The $\mathsf{round}_2(a, n) \,, a \in \mathbb{R} \,\text{and}\, n \in \mathbb{Z}$ in Algorithm~\ref{flpsimfxp} means rounding off all bits after $n$ bits behind the decimal point to $0$.

        \begin{algorithm}[t]
            \setstretch{1.05}
            \SetKwInOut{Input}{\textbf{Input}}\SetKwInOut{Return}{\textbf{Return}}
            \caption{$\mathsf{FLPsimFXP}(x, f, n)$}
            \Input{$x \in \mathbb{R}$ and $\langle n,f \rangle$, defining the representaion format of specific FXP system.}
            \Return{$x \in \mathbf{R}_{\langle n,f \rangle}$.}
            $x \leftarrow \mathsf{OverflowR}(x, n, f)$ \;
            $x \leftarrow \mathsf{UnderflowR}(x, f)$ \;
            $x \leftarrow \mathsf{round}_2(x, f)$ \;
            Return $x$
        \end{algorithm}~\label{flpsimfxp}

    \end{itemize}

    \para{2) \textit{Representation Magnification Factor.  }} Comparing with FLP, the representation range of FXP is extremely limited. For the numerical approximation task, the coefficients tend to be too small to be loaded in FXP systems, especially the coefficients of high-order terms.  

    \begin{remark}[The absolute value of coefficients tend to be small for high-order items in polynomial approximation]~\label{coeff-order}
        Like the rule illustrated in Taylor's theorem, the approximation of $F(x)$ can be expanded as $F(x) = \sum_{n=0}^{\infty}{\frac{F^{(n)}(a)}{n!}(x-a)^{n}}$ around point $a$, the coefficient of $n$-th item is inversely proportional to $n!$. For exponent function $F(x) = a^{x}, a > 1$ whose $n$-th order derivative $F^{(n)}(x) = a^{x}\ln^{n}(a)$, the $n$-th order coefficient in Taylor's expansion is $\frac{a^{x}\ln^{n}(a)}{n!}$, which convergences to 0 when $n \rightarrow \infty$. Actually, the increasing rate of commonly-used real world non-linear functions are lower than exponent function. This phenomenon is consistent with our experiments even the approximation method is not Taylor's expansion, the absolute value of coefficients tend to be tiny for high-order terms. 
    \end{remark}
    
    Such existence of tiny coefficients will demage its precision severely when transformed from FLP to FXP: 1) for coefficients whose absolute value are less than $2^{-f}$, the item will be zero for any order and any large value $x$; 2) though the coefficients are loadable in FXP system (with value larger than $2^{-f}$), the significand are still got severely demaged and cause huge deviation in the high-order item. Take the $8$-th item computation in a $10$-order polynomial approximation of $\mathsf{sqrt}$\footnote{Polynomial $p \in P_{10}$ constructed through the ordinary least square method, within interval $[0, 100]$}, with coefficient transformed from double precision FLP to $<96, 48>$ FXP as an example. The $8$-th item $t_{7}$ for value $x = 100$ is $t_{7}(100) = c_{(p, 7)} \times x^{7} = -1.0435e-11 \times 100^{7}$, Figure~\ref{data example} demonstrate the difference in two environments. The precision are severely demaged for tiny coefficients transformation.
    
    
    % which is in the representaion range of target FXP system($> 2^{-48}$), Figure~\ref{data example} demonstrate this transformation. 
    
    % Such transformation will severely demage the calculation of high-order items especially for large absolute $|x|$. Take $x = 99$ as an example, the evaluated $c_{7}*x^{7}$ with FLP$(c_{7})$ is $-972.64$ while is $-973.08$ with FXP$(c_{7})$, causing unignorable error. This error get worse with smaller coefficient, larger absolute $|x|$ and higher order.

    \begin{figure}[htb]
        \flushright
        \subfigure[FLP example]{
            \label{Floating-point example}
            \includegraphics[width=0.45\textwidth]{./graph/example-FLP.pdf}
        }
        \subfigure[FXP example]{
            \label{Fixed-point example}
            \includegraphics[width=0.45\textwidth]{./graph/example-FXP.pdf}
        }
        \caption{Data Representation Example}\label{data example}
        \flushleft
        \rule{1cm}{0.2mm}
        \fnote{* For clear demonstration, we transform the binary base to decimal. In Figure~\ref{Floating-point example}, as exponent $E = e - 1023$ in double precision FLP, the upper $E = -11$ and the bottom $E = 3$.}
    \end{figure}
    
    Inspired by~\cite{micikevicius2018mixed}, who suffers from precision loss when trying to transform the computation on $32$-bit FLP to $16$-bit, the problem to be addressed is similar in our cases. Figure~\ref{data example} demonstrates the motivation of our method. There is a lot of unused space in FXP after tiny coefficients transformation, and the space still exists after the multiplication with high-order items($100^{7}$ in demonstration). We can left-shift the tiny coefficients by multiplying a factor, letting as much as possible significand loadable in the FXP format, and then multiply the reciprocal of that factor to gain the correct result. For correct evaluation in the FXP environment, we require: 1) the magnified polynomial item can not overflow; 2) the reciprocal of the magnification factor is representable, and 3) the magnification factor should be larger than $1$. We refer to the factor satisfying the above requirements as \textit{Representation Magnification Factor}($s$). We construct the valid $s$ for the $k$-th item evaluation $c_{(p, k)} \times x^{k}$ as:
    \begin{equation}
        s = \min{(2^{f}, \mathsf{FLPsimFXP}^{-1}(\frac{c_{(p, k)} \times x^{k}}{2^{n-f-1}}), 1)}
    \end{equation}
    Such constructed fator $s$ can guarantee gain better evaluation result comparing with only transforming coefficients $c$.
    \todo{proof}

    \para{3) \textit{Residual Boosting}} For $k$-order polynomial $p_{k}(x) = \sum_{i=0}^{k}(c_{(p_k, i)} \times x^{i}) $ approximating function $F$ constructed in the FLP environment, after transformation of tiny coefficient $c_{(p_k, i)}$, there tend to be an unignorable derivation between the origional approximation $p_{k}$ and the new approximation $p'_{k}(x) = \sum_{i=0}^{k}(\mathsf{FLPsimFXP}(c_{(p_k, i)}) \times x^{i})$. We refer to the gap between function $F$ and $p'_{k}$ as \textit{Residual Function} $R$, defining as $R = F - p'_{k}$. Figure~\ref{residual-func} demonstrates the relationship among $F$, $p_{k}$, $p'_{k}$ and $R$. Owing to precision loss, there exist an improvement space for $p'_{k}$ even it is the transformation from a theoretically optimial $p_{k}$ constructed in FLP environment(\eg{the ordinary least square method optimizing the mean squared error}). 
    
    Motivated by Remark~\ref{coeff-order}, we try to use another lower-order polynomial $p_{k-1} = \sum_{i=0}^{k-1}(c_{(p_{k-1}, i)} \times x^{i})$ approximating the residual function $R$, as lower polynomial may suffer less precision loss after the coefficients transformation. As there lack of guarantee that boosting $p'_{k}$ and $p'_{k-1}$ offer better approximation to $F$ comparing with $p'_{k}$ only, here we first check and then boost it to $p'_{k}$ if there exist benefit for approximation. Such procedure can repeat $k$ times till there are no lower polynomial exist (the lowest polynomial is $p'_{0}$ which only have a constant item). We refer such $k$ times check-then-boost procedure as \textit{Residual Boosting}, the formal description is in Algorithm~\ref{residual-boosting}.

    \begin{algorithm}[hbt]
        \normalem
        \setstretch{1.1}
        \SetKwInOut{Input}{\textbf{Input}}\SetKwInOut{Return}{\textbf{Return}}
        \SetKwFunction{boost}{Boost}
        \caption{\textit{Residual Boosting}}
        \Input{Objective function $F$, input domain $[a, b]$, FXP representation $\langle n,f \rangle$, target order $k$, polynomial approximation method $\mathsf{FM}: p_{k} \leftarrow \mathsf{FM}(F, [a, b], k)$ in FLP environment and its error metric $d_{\mathsf{FM}}$.}
        \Return{$p^{*}_{k}(x) = \sum_{i=0}^{k}(\mathbf{c}_i \times x^{i}) \in P_{k}$ with all the coefficients $\mathbf{c}_{i} \in \mathbf{R}_{\langle n,f \rangle}$.}

        \BlankLine
        $p_k \leftarrow \mathsf{FM}(F, [a, b], k)$ \;
        $p^{*}_{k} \leftarrow \sum_{i=0}^{k}(\mathsf{FLPsimFXP}(c_{(p_k, i)}, n, f) \times x^{i})$ \;
        $R \leftarrow F - p^{*}_{k}$ \;
        \For{$k' \leftarrow k-1$ \KwTo $0$}{
            $p_{k'} \leftarrow \mathsf{FM}(R, [a, b], k')$ \;
            $p'_{k'} \leftarrow \sum_{i=0}^{k'}(\mathsf{FLPsimFXP}(c_{(p_{k'}, i)}, n, f) \times x^{i})$ \;
            $p^{tmp}_{k} \leftarrow $ \code{Boost}$(p^{*}_{k}, p'_{k'})$\;
            \tcc{Boost when benefit exist. }
            \If{($|F - p^{tmp}_{k}|_{d_{\mathsf{FM}}} < |F - p^{*}_{k}|_{d_{\mathsf{FM}}})$}{
                $p^{*}_{k} = p^{tmp}_{k}$ \;
                $R = F - p^{*}_{k}$ \;
            }
        }
        \Return{$p^{*}_{k}$}
        \BlankLine
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\boost{$p_k \in P_{k}$ ,$p_{m} \in P_{m}$}}{
            % \BlankLine
            $o \leftarrow \max{(k, m)}$; $p \leftarrow p_{\max{(k, m)}} $ \;
            $p_{o}(x) = \sum_{i=0}^{\min{(k, m)}}(\mathsf{FLPsimFXP}(c_{(p_k, i)} + c_{(p_m, i)}, n, f)\times x^{i}) + \sum_{i=\min{(k, m)}}^{o}(c_{(p, i)} \times x^{i})$ \;
            \Return{$p_{o}$}
        }
    \end{algorithm}~\label{residual-boosting}

    \begin{figure}[b]
        \centering
        \includegraphics[width=0.45\textwidth]{./graph/residual_func.png}
        \caption{Schematic disgram of the \textit{Residual Function}}\label{residual-func}
        \flushleft
        \rule{1cm}{0.2mm}
        \fnote{* Case shown in this figure is a $8$-order approximation of $\mathsf{sqrt}$ within $[40, 80]$ and coefficients transforming from double precision FLP to $<96, 48>$ FXP.}
    \end{figure}

==> revision.tex <==
\section{Revision Statement}\label{sec:revision}

We really appreciate all the constructive comments and suggestions from the reviewers and chairs.  We provide a summary of revision points targeting each comment, and the lines in the margin indicate the changes in the paragraphs.

\subsection{META(R1): Evaluation Clarification}

    \para{Suggestion: } \textit{Clearly connect results with security guarantees (e.g., semi-honest vs malicious). Ack that this contribution is independent of those, but it's hard to talk about MPC performance without guarantees. The paper needs to be self-contained, and its unclear from reading the text whether protocols like Rep2k or RepF are semi-honest or malicious.}

    \para{Revisions: } 
    % We mark the revision for this suggestion in \revise{blue text}.

    1) We briefly introduced the different security assumptions (semi-honest vs. malicious) of each protocol and briefly introduced each protocol in Section~\ref{settings} to make our paper self-contained.

    2) As a readability improvement, we sorted the MPC settings in the evaluation according to their security assumptions (semi-honest first, then malicious) in Table~\ref{Tab:settings}, and adjusted the order for all results accordingly (Table~\ref{Tab:mb-activation} and~\ref{sec:full-microbenchmark}). 

    3) We added an analysis of the performance patterns of \sysname comparing semi-honest vs. malicious in Section~\ref{micro-benchmark}.
    

\subsection{META(R2): Parallelism Experiments}\label{revision:meta-r2}

    \para{Suggestion: } \textit{Scale up parallelism experiments to at least 4 threads, preferably 8.}

    \para{Revision: } 

    To avoid confusion about the kinds of ``parallelism'', we separated the discussion about the following two cases, with separate evaluations and figures to present the results:
    
    1) We added a parallelism evaluation for large vectors using up to 16 threads in Section~\ref{micro-benchmark} (Figure~\ref{Fig:multi-thread}), showing 10 threads achieve the maximum speedup.

    2) We changed paragraph titles in both Section~\ref{sec:oppe} and Section~\ref{micro-benchmark} to separately discuss the case of exploiting the independence of $\times$ and $>$, and the case of parallelizing vector input evaluation.

    % 2) We added a parallelism evaluation for large vectors using up to 16 threads in Section~\ref{micro-benchmark} (Figure~\ref{Fig:multi-thread}), showing 10 threads achieves the maximum speedup. 

    % 2) We changed paragraph titles in both Section~\ref{sec:NFCG-pkm} and Section~\ref{micro-benchmark} to separately discuss the case of exploiting the independence of $\times$ and $>$, and the case of parallelizing vector input evaluation.
    
    % 2) We added a parallelism evaluation for large vectors using up to 16 threads in Section~\ref{micro-benchmark} (Figure~\ref{Fig:multi-thread}), showing speedup up to 10 threads. 
    
 

    % We highlight the revision for this suggestion in \rthread{orange text}.

\rsecurity{
\subsection{META(R3): Security Analysis of NFGen}\label{revision:meta-r3}

    \para{Suggestion: } \textit{The algorithm for obliviously evaluating non-linear functions appears to be constructed under semi-honest assumptions because it assumes all received shares are valid and consistent. Add an end-to-end security proof to show that even if there exist malicious nodes that submit invalid shares or try to prevent honest users from submitting their valid shares, the algorithm can still proceed with correct results and ensure obliviousness. Or describe what happens in the event of a malicious party.}
    
    \para{Revision: } 
    
    % We did not give a clear definition of the security property of \sysname in the original version which raise some misunderstandings. 
    We added the following definitions / analysis / proofs about the security:
    
    1) added a security analysis section (Section~\ref{sec:overview-security}) talking about the security property of \sysname (the behavior in malicious cases were described in the last paragraph); 
    
    2) given the security property definition as well as a proof sketch in Appendix~\ref{sec:formal-security}; 
    
    3) added a more clear definition about obliviousness and analysis in Section~\ref{sec:oppe} and Appendix~\ref{appendix:oblivious-oppe}, following existing works~\cite{hamada2014oblivious} and~\cite{keller2014efficient}.
    
    4) added brief background introductions about common MPC security properties, adversarial models and the real-ideal paradigm in Section~\ref{sec:overview-security} and Appendix~\ref{sec:formal-security} to make the paper better self-contained. 

    In a nutshell, the above new paragraphs of security analysis explains that \sysname's security is equivalent to the underlying MPC protocols it uses, on different kinds of adversarial models / assumptions (including the existence of malicious parties).
    This equivalence is a direct result of \emph{Canetti's composition theorem}~\cite{canetti2000security} since \sysname generates protocol by \emph{modular composing} sub-protocols without revealing any information nor introducing any interaction.
    % For examples, if the subroutines have the property of \emph{guaranteed delivery}, the generated overall protocol also guarantees; if the security property of the subroutines is \emph{secure with abort}, the overall protocol will abort if and only if the abortion happen inside the subroutines.

%    We explain the concerns about \sysname in the following:
%
%    1) For concern about security assumptions (semi-honest assumption and behavior in malicious cases), \sysname preserves the same security property with the three subroutines addition, multiplication and greater-than provided by the underlying MPC platform without introducing any extra assumptions about the adversary model.
%    
%    
%    The above security preserving property is guaranteed by \emph{Canetti's composition theorem}~\cite{canetti2000security} since \sysname generates protocol by composing the three provided subroutines in the standard \emph{modular composition} way~\cite{canetti2000security}, without revealing any information nor introducing any interaction among parties.
%    
%    
%    For examples, if the subroutines have the property of \emph{guaranteed delivery}, the generated overall protocol also guarantees; if the security property of the subroutines is \emph{secure with abort}, the overall protocol will abort if and only if the abortion happen inside the subroutines.
%    % then the abortion may also happen in the overall protocol (inside the subroutines). 
%    The above security analysis and the corresponding proof sketch have been added in a new section (Section~\ref{sec:overview-security}) and Appendix~\ref{sec:formal-security}, respectively.
%    % We add a new section (Section~\ref{sec:overview-security}) talking about the above security analysis and give the corresponding proof sketch in Appendix~\ref{sec:formal-security}.
%    % the security analysis in Section~\ref{sec:overview-security} and give the proof sketch in Appendix~\ref{sec:formal-security}.
%    
%    % the oblivious non-linear function evaluation Algorithm~\ref{Algo:OPPE} keeps the same assumption about the adversary model as the composed three subroutines addition, multiplication as well as greater-than provided by the underlying MPC platform.
%    % \sysname generates the overall evaluation protocol by composing three subroutines addition, multiplication as well as greater-than provided by the underlying MPC platform in the standard \emph{modular composition} way~\cite{canetti2000security}. By Canetti's \emph{composition theorem}~\cite{canetti2000security}, the composition of secure sub-protocols results in secure overall protocol.
%    % We add the security-preserving property analysis in Section~\ref{sec:overview-security} and give the proof sketch in Appendix~\ref{sec:formal-security}.
%
%    % 2) For concern about the malicious cases, the generated evaluation protocol of \sysname achieves the same security property as the provided subroutines in the presence of malicious parties. 
%    % If the subroutines have the property of \emph{guaranteed delivery}, the generated overall protocol also guarantees; if the security property of the subroutines is \emph{secure-with-abort}, then the abortion may also happen in the overall protocol (inside the subroutines). 
%    % Note that all the evaluations except the three subroutines are local computations of each party, no security concerns (revealing no information nor introducing any interaction among parties) are introduced. The revision is the same as the first concern, we further add the examples above in Section~\ref{sec:overview-security} for better illustration.
%
%    2) For concern about obliviousness, the oblivious algorithm in multi-party computation refers to an algorithm design logic, organizing each secure subroutine in an input-independent sequence without branches based on any ciphertext, just like \emph{oblivious sort algorithm}~\cite{hamada2014oblivious} and \emph{oblivious data access algorithm}~\cite{keller2014efficient}.

    % The oblivious algorithm in multi-party computation means each secure subroutine is organized in a deterministic sequence and there are no branches based on the input or any variables directly or indirectly computed from the input like oblivious sort algorithm~\cite{hamada2014oblivious} and oblivious data access algorithm~\cite{keller2014efficient}.

}

\subsection{Other Revision Requirements in Rebuttal}

    % We mark the revision for these suggestions in \rebuttal{teal text}.

\para{1) RA-C1} \textit{You may want to clarify the novelties and contributions in this paper. When I first read the introduction section, I felt like this paper is incremental to some existing efforts that approximate non-linear functions with polynomials. It wasn't until I read enough technical details that I realized that this paper actually makes many optimizations that are tailored for secure computations. Therefore I suggest bringing up some technical contributions to the introduction section and highlighting the significance of these optimizations or improvements. For example, you can have a sub-section in the introduction or an overview section after the intro that (i)formulate the primary research objectives; (ii) summarize key technical contributions; (iii) elaborate on why these optimizations are non-trivial extensions of existing efforts. (some of the discussion may have been included in the introduction, but it might be better to reorganize it.).}

\textbf{Revision: } 

We reorganized part of the introduction (Section~\ref{sec:intro}) by separating it into several parts with subtitles, and highlighted the key challenges and our key ideas. The revised introduction includes:

\begin{enumerate}
	\item current pitfalls;
	\item key challenges;
	\item overview of our key ideas;
	\item summary of key evaluation results;
	\item contributions.
\end{enumerate} 

\para{2) RA-C2} \textit{A (sketch) proof of the obliviousness of the OPPE algorithm should be included. This is currently missing in the paper.}
    
\textbf{Revision: }  

(as part of META-R3 (Appendix~\ref{revision:meta-r3})) We added the proof sketch of the obliviousness with a detailed analysis in Appendix~\ref{appendix:oblivious-oppe}, mentioned in Section~\ref{sec:oppe}.

% We add a more clear definition of the obliviousness of OPPE Algorithm in Section~\ref{} and add the proof sketch with detailed analysis in Appendix~\ref{}.

% We add the proof about the obliviousness property of OPPE Algorithm~\ref{Algo:OPPE} in Theorem~\ref{theorem:oblivious} and mention it in Section~\ref{sec:oppe}.

% We add a more clear definition of the obliviousness of OPPE Algorithm in Section~\ref{} and add the proof sketch with detailed analysis in Appendix~\ref{}. 

% We add the proof about the obliviousness property of OPPE Algorithm~\ref{Algo:OPPE} in Theorem~\ref{theorem:oblivious} and mention it in Section~\ref{sec:oppe}.

% We add a paragraph in Section~\ref{} to introduce some key properties of OPPE Algorithm~\ref{Algo:OPPE}. The proof of obliviousness is in Appendix~\ref{}.

\para{3) RA-C3} \textit{In Table 2, the nonlinear function being evaluated assumes different domains for xx. What is the rationale for choosing these different domains?}

\textbf{Revision: } 

We added the reason at the beginning of Section~\ref{micro-benchmark}.
The input domain of each function in evaluation is set to the interval without a close-to-zero derivative, as these intervals are hard to approximate while others can be simply approximated with some constants. 

\para{4) RA-C4} \textit{The multi-threaded acceleration evaluation was evaluated with only two threads. What would the result (Figure 2) look like if more threads were used (i.e. 4, 8, 16)?}

\textbf{Revision: } 

(as Meta-R2 (Appendix~\ref{revision:meta-r2})). We have added the parallelism evaluations with more threads ($1$ - $16$ threads).

\para{5) RA-C5} \textit{ I don't think Figure 3 illustrates the evaluation results very well, or at least I don't have an idea of the error distribution yet. Maybe it would be much better to use PDF instead of CDF? Another way to show the results is to visualize them with boxplots.}

\textbf{Revision: } 

We provided more quantitative descriptions in Section~\ref{exp:accuracy} to help the readers understand the results in CDF.  In fact, as the percentage of samples with errors below some threshold is a more important metric we want to show, we use CDF which can better show the percentage of low-accuracy samples compared to PDF.


\para{6) RA-C6} \textit{On page 10, you mention "accuracy loss in secret sharing". What are the main causes of this loss of accuracy? If this is a common problem and has been studied in previous work, then citations should be included. If this accuracy loss was found by this study, then you need to explain what caused this accuracy loss.}

\textbf{Revision: } 

This is a common problem as secret-sharing platforms approximate each real value in fixed-point shares, we added the corresponding citations in Section~\ref{exp:accuracy}.

% We still use CDF since the percentage of low-accuracy samples is a more important metric we want to show, which CDF 

% In fact, as CDF better shows the percentage of samples with errors below some threshold compared to PDF, as the percentage of low-accuracy samples is a more important metric we want to show. 


% In fact, as CDF better shows the percentage of samples with errors below some threshold compared to PDF 

% the percentage of low-accuracy samples is a more important metric we want to show

% In fact, we still believe CDF better shows the percentage of samples with errors below some threshold, compared to PDF, as the percentage of low-accuracy samples is a more important metric we want to show. 


% \para{6) RC-Question} \textit{Referring again to Table 2, the time to fit a polynomial is measured in seconds. Meanwhile, the time for direct evaluation is at least an order of magnitude faster for systems A \& F (as is the time for evaluating the fitted polynomial). Is it always the case that the overhead is worth it? Put another way, is it plausible for there to be enough combinations of functions F and domains [a, b][a, b] in a real-life application that the fitting time becomes noticeable?} 

% \todo{find place to add some quantitative descriptions of the benefits = =}

\para{7) RB-W4} \textit{Results are hard to interpret - why not plot NFGen and baselines on the same graph? Tables are harder to grok too.}

\textbf{Revision: }

We highlighted some key results including the speedup and communication save in Table~\ref{Tab:mb-activation} and ~\ref{sec:full-microbenchmark}. For Figure~\ref{Fig:problem-examples}, we plot them separately as there are orders-of-magnitude differences in the errors ($10^{-3}$ vs. $10^{14}$).


\para{8) RC-C1} \textit{In Sec. 4.2, consider explaining Issues 1-3 as they arise (since the reader will have better context) instead of up front.}

\textbf{Revision: } 

We highlighted the related issues at the beginning of each step to make it more clear in Section~\ref{sec:single-poly}.  We separate discussion about issues from the solution, as the relationship is not one-on-one (one solution may help solve multiple issues). 


\para{9) RC-Q1} \textit{Regarding the evaluations of protocol accuracy (Table 2), the comparisons are entirely against the one baseline.}

\textbf{Revision: } 

The \textit{sigmoid}s we adopted are platform's built-in functions and we highlighted them in the beginning of Section~\ref{micro-benchmark}. 

% (we will highlight them in text) and we also compare NFGen with other two related works in Section6.4, showing NFGen achieves better accuracy.
% As we discussed in Section~\ref{sec:single-poly}, the issues arise since the range and resolution of fixed-point are limited, so we put it just after the FXP 
% The issues are caused by the limited range and resolution of fixed-point as we discussed, which are the challenges that all the steps trying to solve, the relationship between issues and steps are not point-to-point.
% \todo{think...}

